Lucky imaging: beyond binary stars

Lucky imaging is a technique for high resolution astronomical imaging at visible wavelengths, utilising medium sized ground based telescopes in the 2--4m class. The technique uses high speed, low noise cameras to record short exposures which may then be processed to minimise the deleterious effects of atmospheric turbulence upon image quality. The key statement of this thesis is as follows; that lucky imaging is a technique which now benefits from sufficiently developed hardware and analytical techniques that it may be effectively used for a wide range of astronomical imaging purposes at medium sized ground based telescopes. Furthermore, it has proven potential for producing extremely high resolution imaging when coupled with adaptive optics systems on larger telescopes. I develop this argument using new mathematical analyses, simulations, and data from the latest Cambridge lucky imaging instrument.

==> ch_aniso/aniso.tex <==
\chapter{Anisoplanatism and the point spread function in lucky imaging}
\label{chap:aniso}


==> ch_calibration/old_doc_chopped.tex <==




\subsection{Taking and Analysing EMCCD Calibration Data}
\label{sec:calibration}
% \subsubsection{Use of pixel histograms in calibration}
\begin{figure}[htp]
\begin{center}
 \includegraphics[width=1\textwidth]{fitted_hist}
\caption[Calibration Frames Histogram]{A histogram of pixel values in 3000 dark frames (with a small light flux due to amplifier glow) taken with the Cambridge CCD. Heavy coloured lines denote regions selected by the algorithm described in text for parameter fitting. Dashed line denotes sum of fitted models. Note excess around the knee of the curve due to serial register CIC electrons.}
\label{fig:histogram}
\end{center}
\end{figure}

When calibrating an EMCCD detector the most useful dataset is a histogram of many pixel values, since this allows us to probe the underlying probability distributions to which the stochastic output conforms. The calibration frames should be taken with a small incident photon flux, so that in each frame there is a chance that a pixel will capture a single photo-electon, but the chance of 2 photo-electrons arriving in the same pixel in a single frame is very small.

Figure~\ref{fig:histogram} shows a histogram from just such a dataset. The general shape of the histogram results from the summation of 2 simple curves: a gaussian distribution curve (centred about 800 DN in this case) and an exponential decay curve (straight line in this linear-log plot) which is truncated at a minimum value slightly larger than the mean value of the gaussian distribution. These are simply explained - pixels are either dark, in which case the photo-electron value before readout is zero, or they have received one photon, in which case the photo-electrons are multiplied by the serial register, resulting in a value stochastically distributed along an exponential decay curve \citep{Matsuo1985, Basden2003}. These photo-electron values are then converted to data numbers by the readout mechanism, which adds a bias pedestal (800 DN in this case) and some readout noise which is well approximated by a gaussian. So the histogram represents a single peak at 0, and an exponential tail, both of which have been shifted by 800 and then convolved by a gaussian:

\begin{equation}
\begin{split}
 P(x)\ = \ P(N_{phot}=0)\times\texttt{GaussianRO(mean bias, RO noise)}  
\\
  + \ P(N_{phot}=1)\times\texttt{Convolution[ Exponential(Gain)*GaussianRO ]}
\end{split}
\end{equation}

(Equation to be properly expressed mathematically in final version)\\
Clearly, by fitting the parameters of this model to the histogram we can infer the absolute value of the photo-electron flux, the bias pedestal level, the readout noise and, crucially, the mean gain level. 


In practice, there are complications - bad pixels produce values that do not conform, and if the light level is chosen to produce a reasonable proportion of light pixels then the chance of 2 photons arriving in one pixel exposure will be small but possibly non-negligible. There is also the issue of clock induced charge (CIC, see section~\ref{sec:CIC}) - charge induced during frame transfer will result in the same distribution of pixel values as regular photo-electrons, but charge induced in the serial register will not undergo the same number of multiplication stages, and therefore will conform to a different exponential distribution with a mean gain equal to the square root of the mean gain experienced by photo-electrons (C.D. Mackay, private communication). It is this serial register CIC which results in the excess of the histogram above the knee of the fitted curve, since the lower gain for these electrons results in a steeper exponential slope.


The algorithm used to determine the parameters is conceptually very simple, and consists of a multi-stage fitting process - first 
% the mean and readout sigma of the gaussian are estimated from the mode and width at half maximum of the histogram, then 
a gaussian curve is fit by a least squares routine to the region left of the peak (heavy blue section in figure~\ref{fig:histogram}) where there should be no contamination from illuminated pixels. Second, the exponential is fit. This region of fit must be far enough from the gaussian peak so that it only includes a negligible count of ``dark'' pixels, rejects most serial register CIC pixels, and should terminate before reaching very low and therefore noisy pixel counts (heavy blue section in figure~\ref{fig:histogram}). Exact details of the algorithm can be found in the source code.
% In practice we find that a region which is chosen to range from 3.5$\sigma$ above the gaussian mean, and terminates at the larger of 100 pixel counts, or 1 millionth of the maximum pixel count, works well (heavy green section in figure~\ref{fig:histogram}).
%  (Need to check those limits in the code). 

The algorithm is implemented in C++, making use of the ROOT Minuit2 minimization library 
\footnote{Available from http://seal.web.cern.ch/seal/work-packages/mathlibs/minuit/index.html}, 
and source is available from (link to own website). We note an independently developed routine of similar purpose by \cite{Daigle2009} for IDL is available from (link) - but a comparison is beyond the scope of this paper.
%  but we hope they prove complementary, and user choice between them will most likely depend on the programming environment in use.

In theory it would be possible to calibrate the detector by performing histogram fitting on a pixel by pixel basis, but to ensure an accurate fit for each pixel this would require tens of thousands of dark exposures obtained under very stable gain and temperature. It is more practical to characterise the detector using knowledge of the characteristics as described below.


\subsection{Bias Level and Readout Noise}

\begin{figure}[htp]
\begin{center}
 \includegraphics[width=0.8\textwidth]{bias_temporal_var}
\caption[Temporal Bias Variation]{Temporal bias variation in the Cambridge summer 2009 data}
\label{fig:temporal_bias_variation}
\end{center}
\end{figure}

\begin{figure}[htp]
\begin{center}
 \includegraphics[width=0.8\textwidth]{bias_plot}
\caption[Column to Column Bias Variation]{Column to column spatial bias variation in the Cambridge summer 2009 data. Note that the spike at column 628 is due to a column of bad pixels.}
\label{fig:col_bias_variation}
\end{center}
\end{figure}
As with a conventional CCD the readout for a dark pixel has a mean value equal to the bias offset or 'pedestal.' This offset is typically at a value of around 700-800 data numbers. 

The Cambridge detector has both a column to column variation in the bias level, as depicted in figure~\ref{fig:col_bias_variation}, and a small temporal variation which appears to be uniform across the detector (Figure~\ref{fig:temporal_bias_variation}). Analysis of long datasets from the summer 2009 data suggests that the spatial column bias variation pattern is stable to within $\pm1.5$ data numbers for a fixed gain, once the temporal variation across the CCD has been removed. The temporal variation is not immediately evident in a summed image due to its uniformity, but will blur the pixel histograms used to determine gain value, etc. and so should be corrected as far as possible to ensure accurate measurement. The temporal bias variation can be measured by histogram fitting for each frame, or less accurately but with less computational effort by taking the mode of the pixel values in each frame.0

The spatial bias pattern varies with gain (figure x). Therefore, to correct for the spatial variation in fields which are crowded or otherwise have high background flux variation, a bias calibration frame must be separately obtained for each gain setting to be utilised. The simplest method of obtaining this bias calibration frame is from a series of dark exposures - after summing the frames to obtain an average, a sigma clipped mean value for each column is used to estimate the bias offset\footnote{Note that this assumes the dark frames are vertically uniform - it therefore best to take a mean over the values above row 200, since the amplifier glow results in non-uniformity below - see section~\ref{sec:dark_level}. }.
However, for a large dataset consisting of a sparsely populated field of view with no bright stars and low background, calibration can be obtained directly from the sky data by taking a histogram for each column across all the exposures, since this will give enough dark pixels for histogram fitting to determine the bias offset with good accuracy. Of course, this requires an extra reduction stage of the data to obtain the bias frame prior to the main reduction.

Alternatively, data reduction of sparse fields can be performed in a single pass without a pre-existing bias frame by simply subtracting the mode of each column from every pixel in that column, frame by frame. The loss of accuracy that results from such small histogram samples results in a small difference in the average bias frame applied, typically less than 2 data numbers across most of the CCD (Figure~\ref{fig:bias_methods}).

\begin{figure}[htp]
\begin{center}
 \includegraphics[width=0.8\textwidth]{bias_methods}
\caption[Comparison of bias calibration methods]{A comparison of the bias calibration methods as described in the text.}
\label{fig:bias_methods}
\end{center}
\end{figure}

As with a conventional CCD the readout process is noisy, and the spread in pixel values is well modelled by a Gaussian distribution. The RMS (after correcting for bias variation)
% can be determined from fitting of a pixel histogram (see \ref{sec:reduction}), and 
is typically 10 data numbers in the summer 2009 data. This results in an RMS value of 0.11 photo-electrons per pixel per frame for a typical gain of 90DN per photo-electron when using the data in analogue mode. Thresholding (Section~\ref{sec:thresholding}) lowers this RMS further.


\subsection{Dark Level}
\label{sec:dark_level}
In the context of a well cooled, high frame rate, high gain EMCCD ``dark current'' is dominated not by thermal emissions as with a conventional CCD, but rather clock induced charge and amplifier glow.

\subsubsection{Clock Induced Charge}
\label{sec:CIC}
There is always a slim chance that a pixel which has not received any photo-electrons will still result in a non-zero electron level at readout, due to an electron being randomly dislodged at some point of the stochastic gain serial register, or during the frame transfer (best reference?). Tests with the Cambridge group EMCCD suggest serial register dark electrons are the most frequent (C.D. Mackay, private communication). As a result of such electrons only dislodging part way through the gain register, the clock induced charge generally has a much lower average gain than the photo-electrons (although this is not the case for stray electrons introduced during frame transfer). There are preliminary results to suggest that CIC levels vary slightly across the CCD area due to the way clock signal edges are damped as they propagate from the edge to the middle of the image and into the store area(C.D. Mackay, private communication). Relative to other noise sources we suspect this effect is negligible but it has not yet been exhaustively characterised.



\subsubsection{Amplifier Glow}
\label{sec:amp_glow}
\begin{figure}[htp]
\begin{center}
 \includegraphics[width=1\textwidth]{amp_glow2}
\caption[Amplifier Glow]{Dark current in the lower 250 rows of debiased dark frames from summer 2009 data. \\Top: Analogue mode.\\ Bottom: Thresholded for photon counting. \\Note the shape of the non-uniformity changes significantly with thresholding, suggesting that the ``dark current'' to the left is actually due to vertical variation in the bias pedestal, while the dark current on the right is probably due to real excess photon flux from the amplifier glow.}
\label{fig:amp_glow}
\end{center}
\end{figure}

\begin{figure}[htp]
\begin{center}
 \includegraphics[width=1\textwidth]{dark_col_plot}
\caption[Dark Current Variation]{A plot of the photon counts in a single column of the dark-current calibration frame illustrates the spatial variation. Plotted are values for analogue mode and with photon counting thresholds applied.}
\label{fig:dark_current_col}
\end{center}
\end{figure}

The summer 2009 data taken with the Cambridge camera shows what appears to be significant amplifier glow in the bottom quarter of the frame, so that below about row 150 this dominates over typical sky and CIC flux - it also adds non-uniformity over most of the frame, as illustrated by the column values plot in figure~\ref{fig:dark_current_col}. The spatial variation is characterised by a curve which looks roughly like exponential decay, but in practice is not simply parameterised, so good calibration flats are essential if dark current patterns are to be removed.

In practice the calibration is further complicated by a small residual variation in the bias pattern in the lower left of the frame, after column debiasing. This can be estimated by comparing dark current frames composed from analogue mode and thresholded data (Figure~\ref{fig:amp_glow}), since the thresholded data is relatively insensitive to the bias offset. 


\cite{Tulloch2004} describes similar noise in a CCD87 detector. It should be noted that although the additional photo-electrons can be calibrated from dark frames and removed, added photon shot noise will remain and should be taken into account when analysing reduced data. 

\subsubsection{Typical Levels of Flux in Dark Frames}
\cite{Tulloch2008} states that typical CIC rates for EMCCD detectors used at the ING are 0.03 electrons per pixel per frame, while \cite{Daigle2009} give a combined dark current plus CIC photon-event rate for an Andor CCD97 camera of 0.0084 electrons per pixel per frame (both for a 10MHz pixel rate). Preliminary analysis of dark frames from the Cambridge 2009 data suggests a combined flux of 0.04 electrons per pixel per frame in areas where the amplifier glow is least. It is unclear at present whether this value is mostly due to CIC, the faint wings of the amplifier glow, or possibly other light leakage.


\subsection{Flat Fielding}
\subsubsection{Gain Variation}
Tests with the summer 2009 data suggest there is a small amount of spatial gain variation, varying smoothly from column to column across the chip. Figure~x shows a typical pattern. The total range of the variation is about 3\%, and so careful calibration is a must for accurate photometry. A long series of dark frames, or on-sky data with only very faint sources across the field, is essential for accurate spatial gain calibration.
 Gain variation over time seems to be well controlled, of the order of less than 1\% per 10,000 frames - however this should be carefully monitored and accounted for when reducing long exposure datasets. (Figure. x)

\subsubsection{Pixel Quantum Efficiency and Sky Exposure}
EMCCDs are no different from regular CCDs in this regard - a sky flat field must be taken to measure variations in pixel efficiency and camera throughput. In theory it should be possible to produce a ``superflat'' by taking the median sky flux of each pixel in thresholded images from many datasets, relative to the typical sky flux in each dataset. However this relies on all other aspects of the calibration process performing well, and in practice a twilight sky flat is much simpler.

Traditionally sky flats have been a source of much contention - for example, it is hard to gauge whether a dust mote blocks the same proportion of light from a bright source as it does from a faint source, and throughput may also vary with filter. One advantage of lucky imaging is that small, severe artifacts can in fact be marked as ``bad pixels'' and drizzled over using values from the adjacent pixels under different tip-tilt dither positions, albeit with a loss of signal-to-noise corresponding to the loss of pixel-exposures.


\subsection{Other Issues}
Previous Cambridge detectors have suffered from single pixel CTE effects - visible as vertical pairs of unusually dark and bright pixels, or  horizontal pairs of a photon-event pixel and a corresponding bright adjacent pixel (circa \cite{Daigle2009} figure 8), however there is no evidence of this issue in the 2009 detector. Unfortunately there were a few ``hot columns'' which are stuck at high values - these were noted and masked during the data reduction process.

When bright sources are incident on the detector some other effects become apparent. The first is an unavoidable artefact of the way a frame is read out - a bright star can be seen to leave a uniform vertical trail of photon-events as the pixel charges are shifted into the frame store. The frame shift period is approx 3\%  of the duty cycle and so the sum flux over the entire column in sky areas will be 3\% of the sum flux in the pixels of that column which are normally under the star position. 
As a result, the per pixel sky-excess from this effect is a factor of $10^{-5}$ smaller than the sum star flux incident upon a single column. This effect can be fairly easily calibrated and subtracted by incorporating a correction into PSF fitting routines, or in sparse fields it may simply be removed by analysing the background field for vertical banding.

The second bright source effect appears to be an artefact occuring somewhere during the readout process. A bright star also creates a horizontal band of raised pixel values, due to poor charge transfer efficiency in the serial direction. This effect appears to be non-uniform, and efforts are ongoing to characterise this effect so it can be reliably subtracted. 

Both the horizontal and vertical trail effects are relatively minor, typically causing an increased pixel flux of less than 0.01 photo-electrons per frame, and are immediately obvious as detector artefacts when visually inspected. As a result, un-calibrated trails only contribute significant errors in lucky imaging data when performing photometry or astrometry of faint stars that occupy the same column or row as a bright star.




\subsection{Recipes}
\label{sec:recipes}
When dealing with a dataset which varies both spatially and temporally in a noisy manner, extracting the underlying patterns of those variations can be difficult. We are faced with a bootstrap problem - do we average spatially, resulting in a histogram which is an accurate representation of a single frame, but, distorted by spatial variation, or gather values over a small area for many frames with distortion from temporal variation? The following are routines we have found effective for our detector:

\subsubsection{Bias, Gain and Dark Current Calibration}

\begin{itemize}
 \item First, a series of dark images should be taken for each combination of gain setting and windowing mode, in order to accurately determine the bias and gain variations. 

\item From each configuration's dark images, a simple average of the dataset should be taken, for a quick inspection of the data. This allows for easy identification of hot columns, bad pixels, etc. For dark frames the dominant spatial variation in a simple average is due to column to column bias variation. Therefore this average can also be used to pick a region where the spatial bias variation is least - usually in the upper right of the detector (Figure~\ref{fig:zeroed}). 

\item The frames are then stepped through, and this region of least spatial variation is used to generate a histogram which can be used to identify the uniform bias level of the current frame. In this way the (spatially uniform) temporal variation in the bias pedestal can be identified and removed .

\item The series of stabilised frames can then be used to generate a histogram for each column which can be used to accurately measure the column to column spatial variations in both bias and gain (Figure~\ref{fig:col_bias_variation}). 

\item The newly determined bias frame and gain flat field correction can then be applied to the dark data to arrive at an average image consisting purely of ``dark current'', and this is used to calibrate the spatial variation in amplifier glow.
\end{itemize}

\subsubsection{Science Data Reduction}
\begin{itemize}
 \item As with calibration data, a quick average of say, 1000 frames should be taken first (this is essential anyway in lucky imaging for choice of guide star). This allows selection of a region free from stars where the photon flux is much less than 1 photon per pixel per frame.
\item The frames are then stepped through by the main reduction loop:
\item If a pre-existing bias correction frame exists, this should be applied to each frame. Otherwise for a sparse field a column-by-column mode correction can be applied.
\item The temporal bias variation should be corrected for, either by fitting a gaussian to, or simply taking the mode of a histogram of pixel values from the frame.
\item Pixel values from the star free region should then be added to the histogram collated over the whole dataset. This can be used to accurately calibrate the gain setting for the run.

\item Thresholding techniques can then be applied using knowledge of the bias and the gain, in a second pass (in lucky imaging it is natural to perform a second pass anyway so that frame selection can be done with knowledge of the full dataset).


\end{itemize}


% \section{Frame reduction routines}
% \label{sec:reduction}

\section{Optimal Thresholding Levels for Photon Counting}
\label{sec:thresholding}

The stochastic nature of the signal multiplication in EMCCDs introduces an extra source of variability, so that compared to the ideal case of purely photon shot noise an EMCCD at high light levels will experience signal variation larger by a factor of $\sqrt{2}$ - this is termed the ``excess noise factor'' \citep{Basden2003}. At low light levels (where the mean photon flux per pixel per frame is much less than 1) we can be reasonably confident that any given pixel only contains 0 or 1 photons. In this case we can exploit the fact that most photon events result in values many times the RMS background noise above the background to reduce this signal variation by employing a pixel thresholding scheme. In the case of low light levels this is referred to as photon counting (PC). Both \cite{Basden2003} and \cite{Lantz2008} have explored the possibility of extending this to higher light levels via either multiple thresholds or Bayesian estimators. However there are a number of practical issues with these schemes. 

Firstly, they require excellent knowledge of the gain level, which must be both well controlled during data acquisition and measured with high precision during data reduction. The scheme of \citeauthor{Basden2003} results in a very low threshold between the bins for zero and one photons, which results in a high sensitivity to detector noise (also CIC effects are unaccounted for by \citeauthor{Basden2003} and hence their effects are unknown). The scheme of \citeauthor{Lantz2008} requires the mean light level on every pixel to be constant so that an optimum Bayesian estimator can be chosen - in application to lucky imaging they suggest thresholding on frames which have been already recentred using the guide star. This is not entirely unfeasible but would be computationally expensive and does not account for anisoplanatic effects.

As a result we have chosen to focus on photon counting methods\footnote{To our knowledge no-one has yet applied high light level thresholding schemes to lucky imaging data in practice.}. As we will show, thresholding is at any rate most needed at low light levels where the detector noise would otherwise dominate over the photon shot and stochastic multiplication noise.

The question of optimum threshold choice for photon counting was partially treated in section 2 of \cite{Lantz2008} but in that paper the authors focused on optimizing the exposure time, and hence light level, alongside the threshold to achieve a minimum ``misfit,'' i.e. to ensure absolute photon count estimations were as close as possible to their true values.
In contrast, we assume that true photon counts can be estimated from the thresholded values, and focus on achieving optimum signal to noise in the thresholded estimate, accounting for the fact that too high a threshold will effectively result in  higher photon shot noise. 

Finally, in lucky imaging data there is always a range of light levels, and so we also explore the effectiveness of applying a single threshold over a range of light levels, relative to the optimum.

\subsection{Assumptions and Basic Equations}
Assume that:
\begin{itemize}
 \item Readout noise follows a gaussian distribution with mean value 0, and variance $r^2$. 
 \item Given one photo-electron input to the serial multiplication register, output data numbers are distributed with probability
\begin{equation}
 p(x) = \frac{e^{-x/g_s}}{g_s} 
\end{equation}
so that 
\begin{equation}
 \sum_{x=1}^{x_{max}}p(x)=1
\end{equation}
where $g_s$ is the ``signal gain'' i.e. the gain experienced by real photon events, and $x_{max}$ is the saturation level.

\item Clock induced charge events occur with frequency $\lambda_{par}$ per pixel per frame during frame transfer, and with frequency $\lambda_{ser}$ during charge transfer in the serial register. Assume they occur in a random process well approximated by a Poisson variate of very low mean. CIC events occurring during frame transfer are read with grey levels distributed in the same way as a single photo-electron.

CIC events originating from the serial register will undergo different levels of gain according to which stage of the register they occur in. However, we can make a first order approximation to the value distribution by assuming an average gain $g_{cic}$, so that serial register events are distributed with probability:
\begin{equation}
 p(x) = \frac{e^{-x/g_{cic}}}{g_{cic}}
\end{equation}
We expect $g_{cic}\approx\sqrt{g_s}$ (C.D. Mackay, private communication).
\end{itemize}

\subsection{Basic signal to noise equation}
We can now construct the basic signal to noise equation relevant to determining the mean photon flux incident on single pixel, from the following components: 
\begin{itemize}
 \item The mean photon flux; $\mu$ (photons per pixel per frame).
 \item The readout noise, which has standard deviation $r$.
 \item The average gain level for a photo-electron (signal gain) $g_s$.
\item The respective frequencies of frame transfer CIC events and serial register CIC events; $\lambda_{par}$ and $\lambda_{ser}$.
 \item The average gain level for a serial register event (serial CIC gain) $g_{cic}$.
\end{itemize}


For a regular, non electron multiplying CCD the standard signal to noise ratio (SNR) equation is typically (neglecting dark current):
\begin{equation}
 SNR = \frac{\mu}{\sqrt{\mu+r^2}} 
\end{equation}
where the readout noise RMS $r$ is typically of the order of a few photo-electrons, but is higher when the CCD is run at high frame rates. From this we can see that at signal levels any lower than 1 photo-electron per pixel per frame the readout noise will dominate over the signal.

For an EMCCD, the data number output for a fixed input of $n$ photo-electrons (i.e. without photon-shot noise) has mean $ng_s$ and variance $ng_s^2$ \citep{Basden2003}. This is added in quadrature to the photon shot noise. We also include the noise due to CIC events. For a mean photo-electron flux of $\mu$ the basic SNR equation then becomes:
\begin{equation}
 SNR = \frac{\mu g_s }{\sqrt{2\mu g_s^2  + 2\lambda_{par}g_s^2 +  2\lambda_{ser}g_{cic}^2  + r^2}} 
\end{equation}
Which we can rearrange as
\begin{equation}
 SNR = \frac{\mu}{ \sqrt{	2\mu   + 2\lambda_{par} +  2\lambda_{ser}\frac{g_{cic}^2}{g_s^2 }  + \frac{r^2}{g_s^2}	} } = \frac{\sqrt{\mu}}{E}
\end{equation}
where $E$ is the excess noise factor relative to an ideal detector. From this equation we can deduce a couple of points. First, at high light levels the photon count dominates over the other terms and $E\approx\sqrt{2} $. Second, at low light levels the dominant noise term will depend largely on the relative magnitudes of $\frac{r^2}{g_s^2}$ and the CIC event frequencies. In practice, for the current generation of EMCCDs CIC events dominate over the readout noise at high enough gain  (typically $\frac{g_s}{r}=10$, $\lambda_{par}=0.03$).

\begin{figure}[htp]
\begin{center}
 \includegraphics[width=1\textwidth]{analog1}
\caption[Analog Signal to Noise]{Signal to Noise at various light levels for an analogue mode EMCCD, relative to the ideal case of purely photon shot noise. This is equivalent to $1/E$. Dashed line denotes high flux asymptote of $1/\sqrt{2}$. Detector parameters used to generate the plot were: $r=1$, $g_s$=10, $g_{cic}$=6, $\lambda_{par}$=0.03, $\lambda_{ser}$=0.01. It is clear that for these detector characteristics analogue mode SNR drops off steeply below flux of about 0.2.}
\label{fig:analog_stn}
\end{center}
\end{figure}


\subsection{Choosing the threshold grey level to achieve best signal to noise}
For sufficiently low flux levels we can assume that the chance of 2 or more photons being incident on the same pixel is small (e.g. for $\mu=0.2$, \mbox{$P(n=2)\approx0.016$}). With this prior condition we can set a grey-level threshold such that pixels are assigned exactly 1 or 0 photons depending on whether the grey-level is above or below the threshold. This processing of the data removes the stochastic multiplication effect, and also cuts out much of the noise resulting from readout variation, but it also lowers the effective light level, and so we look to the signal to noise equation to try and determine the most effective threshold level.

In calculating where to set the grey level threshold $T$, the key additions to the SNR equation above are 
\begin{itemize}
 \item The fraction, $\alpha_s$ of single photon pixels that are above the threshold: \begin{equation}
		\alpha_s = 1 - \sum_{x=1}^{x=T}p(x) \approx e^{-T/g_s} \qquad \qquad \Big[p(x) = \frac{e^{-x/g_s}}{g_s} \Big]
                                                                          \end{equation}
 \item The fraction, $\epsilon$ of zero photon pixels that are counted as photon events due to readout noise:  \begin{equation}
             \epsilon(T/r) = 1 - \Phi(T/r) = \Phi(-T/r)
                                                                                             \end{equation}
where $\Phi(t)$ represents the CDF of a normal distribution.
\item The relative ratio of photon event pixels $(\mu)$ and dark pixels $(1 - \mu)$
\item And the fraction of serial register clock-induced-charge electrons that pass the threshold:
 \begin{equation}
		\alpha_{cic} \approx e^{-T/g_{cic}}
\end{equation}
\end{itemize}

\subsubsection{Thresholded Signal to Noise equation}
Hence; in the thresholded regime we essentially have a reduced mean poissonian flux $\alpha_s \mu$ with variance $\alpha_s \mu$, and a reduced background noise resulting from the occasional CIC events or high readout-noise events that pass the threshold. If we make the assumption that these background noise events can be modelled as low mean poissonian processes with respective mean frequencies of:
\begin{itemize}
 \item $(1-\mu)\lambda_{par}\alpha_s$ for the parallel transfer CIC events,
 \item   $(1-\mu)\lambda_{ser}\alpha_{cic}$ for the serial register CIC events
 \item and $(1-\mu)\Phi(-T/r)$  for the high readout events
\end{itemize}
 then the new SNR equation is:
 \begin{equation}
  SNR=\frac{ \alpha_s\mu}{\sqrt{ \alpha_s\mu +(1-\mu)\big(\lambda_{par}\alpha_s + \lambda_{ser}\alpha_{cic} + \Phi(-T/r) \big) }}
 \end{equation}
\begin{equation}
 = \frac{\sqrt{ \mu }}{\sqrt{ 1/\alpha_s +\frac{(1-\mu)}{\mu \alpha_s^2}\Big(\lambda_{par}\alpha_s + \lambda_{ser}\alpha_{cic} + \Phi(-T/r) \Big)  }}
\end{equation}
Note that the $(1-\mu)$ factor is present because unlike the analogue case readout noise etc. does not affect photon-events that pass the threshold, due to the digitization.
We can then expand the denominator to get the excess noise factor purely in terms of the detector properties and photo-electron flux:
\begin{equation}
 E = \sqrt{e^{T/g_s} + \big(\frac{1-\mu}{\mu}\big)e^{2T/g_s} \Big(\lambda_{par} e^{-T/g_s}+ \lambda_{ser} e^{-T/g_{cic}} + \Phi(-T/r) \Big) }
\end{equation}
Intuitively the problem can be best understood as a case of finding the lowest threshold point at which more signal photons are still being passed than noise photons.


For a given set of detector characteristics (readout rms r, gain level $g_s$, CIC characteristics $\lambda$,$g_{cic}$) we can now go about choosing a threshold level that produces the best signal to noise ratio for a given target brightness n.

\subsubsection{Threshold Optimization for a range of light levels}
\begin{figure}[htp]
\begin{center}
 \includegraphics[width=1\textwidth]{opt_thresh_vals}
\caption[Optimum Threshold Level]{Optimum threshold level over a range of flux levels.}
\label{fig:optimum_thresh}
\end{center}
\end{figure}

Figure~\ref{fig:optimum_thresh} shows a plot of the optimum threshold level over a range of photon-fluxes. Although the optimum threshold varies considerably, the loss of SNR as the threshold is changed from the optimum is actually quite slow. (Could include contour plots of SNR(flux,threshold) - a bit hard to interpret though?) As a result, choosing a single threshold level optimum for a mid-range flux intensity results in near optimum signal to noise over a wide range of light levels, as illustrated in figure~\ref{fig:thresh_comparison}.

\begin{figure}[htp]
\begin{center}
 \includegraphics[width=1\textwidth]{thresh_comparison}
\caption[SNR comparisons]{Comparison of relative signal to noise. Blue dots represent analogue mode. Magenta dots are SNR using optimum threshold level for each flux, while yellow dots (mostly overlaid on the magenta) are SNR for a fixed threshold of 2.65 times the readout RMS (optimal for a flux of 0.1 photo-electrons per pixel per frame). Detector parameters are the same as for figure~\ref{fig:analog_stn}.}
\label{fig:thresh_comparison}
\end{center}
\end{figure}

\subsection{Thresholding results with real lucky imaging data}

\section{Appendix}
\subsection{Mathematica Code}
% The SNR plots were produced using the following Mathematica functions:
% \begin{verbatim}
%  myReadNoisePass[T_, R_] := CDF[NormalDistribution[0, R], -1*T]
% 
%  mySigPass[T_, G_] := Exp[-T/G]
% 
%  mySigtoN[n_, T_, Gs_, Ro_, lambda_, Gcic_] := 
%  n*mySigPass[T, Gs] / 
%    Sqrt[
% 		n*mySigPass[T, Gs]^2 + lambda*mySigPass[T, Gcic ] + (1 - n)*myReadNoisePass[T, Ro]
%         ]
% \end{verbatim}




\bibliographystyle{../bibstyles/hapj}
\bibliography{../bibs/myrefs}

\end{document}


==> ch_science/WASP_companions_table/django_companions_table_template.tex <==




% 
% After creating the table.tex with python,
% include the table.tex in your main.tex file.
% Needs graphicx and a definition of \obs_table_scale
% (see table_placeholder.tex)


%     \begin{tabular}{lllrrrp{3cm}}
 \scalebox{\CompanionTableScale}{
	\begin{tabular}{|l|c|c|c|c|c|c|c|}
	\hline
	 \textbf{Target} & \multicolumn{7}{c|}{\textbf{Companion Parameters}} \\
	\hline
	{% for col in cols_info %}

		\begin{minipage}{ {{ col.0 }}cm }%
		\vspace{1ex}
		\begin{center}
		{% autoescape off %}
		\textbf{ {{col.1.title}} } 
		{% endautoescape %}
		\end{center}
		\end{minipage}

		{% if not forloop.last %}
		&
		{% endif %}
		
	{% endfor %} 
	\\[3ex]
    \hline
		& & & & & \\[-2ex]
    {% for row in  table %}
        {% for entry in row %}
			{% if entry.asymmetric_errors or entry.reg_errors %}
				{% if entry.reg_errors %}
					{{ entry.value }} \raisebox{0.1ex}{ \small{$\pm{{ entry.sym_error}}$ } }
				{% endif %}	
				{% if entry.asymmetric_errors %}
					${{ entry.value }}$ ${ }_{ {{ entry.neg_error}} }^{ + {{ entry.pos_error}}  }$
				{% endif %}
			{% else %}
				{{ entry.value }}
            {% endif %}
            {% if not forloop.last %} 
               &
            {% endif %}
        {% endfor %}
        \\[1ex]
    {% endfor %}
    \hline
    \end{tabular}
} %end scalebox






==> ch_science/WASP_obs_table/django_table_template.tex <==




% 
% After creating the table.tex with python,
% include the table.tex in your main.tex file.
% Needs graphicx and a definition of \obs_table_scale
% (see table_placeholder.tex)


%     \begin{tabular}{lllrrrp{3cm}}
 \scalebox{\ObsTableScale}{
	\begin{tabular}{|lllcccc|}
    \hline
	{% for col in head %}

		\begin{minipage}{ {{ col.0 }}cm }%
		\begin{center}
		\vspace{1ex}
		{% autoescape off %}
		\textbf{ {{col.1}} } 
		{% endautoescape %}
		\end{center}
		\end{minipage}

		{% if not forloop.last %}
		&
		{% endif %}
		
	{% endfor %} 
	\\[3.6ex]
    \hline
    {% for row in  table %}
        {% for cell in row %}
            {{cell}}
            {% if not forloop.last %} 
               &
            {% endif %}
        {% endfor %}
        \\
    {% endfor %}
    \hline
    \end{tabular}
}






==> rgb.tex <==
\definecolor{AliceBlue}{rgb}{0.94,0.97,1.00}
\definecolor{AntiqueWhite1}{rgb}{1.00,0.94,0.86}
\definecolor{AntiqueWhite2}{rgb}{0.93,0.87,0.80}
\definecolor{AntiqueWhite3}{rgb}{0.80,0.75,0.69}
\definecolor{AntiqueWhite4}{rgb}{0.55,0.51,0.47}
\definecolor{AntiqueWhite}{rgb}{0.98,0.92,0.84}
\definecolor{BlanchedAlmond}{rgb}{1.00,0.92,0.80}
\definecolor{BlueViolet}{rgb}{0.54,0.17,0.89}
\definecolor{CadetBlue1}{rgb}{0.60,0.96,1.00}
\definecolor{CadetBlue2}{rgb}{0.56,0.90,0.93}
\definecolor{CadetBlue3}{rgb}{0.48,0.77,0.80}
\definecolor{CadetBlue4}{rgb}{0.33,0.53,0.55}
\definecolor{CadetBlue}{rgb}{0.37,0.62,0.63}
\definecolor{CornflowerBlue}{rgb}{0.39,0.58,0.93}
\definecolor{DarkBlue}{rgb}{0.00,0.00,0.55}
\definecolor{DarkCyan}{rgb}{0.00,0.55,0.55}
\definecolor{DarkGoldenrod1}{rgb}{1.00,0.73,0.06}
\definecolor{DarkGoldenrod2}{rgb}{0.93,0.68,0.05}
\definecolor{DarkGoldenrod3}{rgb}{0.80,0.58,0.05}
\definecolor{DarkGoldenrod4}{rgb}{0.55,0.40,0.03}
\definecolor{DarkGoldenrod}{rgb}{0.72,0.53,0.04}
\definecolor{DarkGray}{rgb}{0.66,0.66,0.66}
\definecolor{DarkGreen}{rgb}{0.00,0.39,0.00}
\definecolor{DarkGrey}{rgb}{0.66,0.66,0.66}
\definecolor{DarkKhaki}{rgb}{0.74,0.72,0.42}
\definecolor{DarkMagenta}{rgb}{0.55,0.00,0.55}
\definecolor{DarkOliveGreen1}{rgb}{0.79,1.00,0.44}
\definecolor{DarkOliveGreen2}{rgb}{0.74,0.93,0.41}
\definecolor{DarkOliveGreen3}{rgb}{0.64,0.80,0.35}
\definecolor{DarkOliveGreen4}{rgb}{0.43,0.55,0.24}
\definecolor{DarkOliveGreen}{rgb}{0.33,0.42,0.18}
\definecolor{DarkOrange1}{rgb}{1.00,0.50,0.00}
\definecolor{DarkOrange2}{rgb}{0.93,0.46,0.00}
\definecolor{DarkOrange3}{rgb}{0.80,0.40,0.00}
\definecolor{DarkOrange4}{rgb}{0.55,0.27,0.00}
\definecolor{DarkOrange}{rgb}{1.00,0.55,0.00}
\definecolor{DarkOrchid1}{rgb}{0.75,0.24,1.00}
\definecolor{DarkOrchid2}{rgb}{0.70,0.23,0.93}
\definecolor{DarkOrchid3}{rgb}{0.60,0.20,0.80}
\definecolor{DarkOrchid4}{rgb}{0.41,0.13,0.55}
\definecolor{DarkOrchid}{rgb}{0.60,0.20,0.80}
\definecolor{DarkRed}{rgb}{0.55,0.00,0.00}
\definecolor{DarkSalmon}{rgb}{0.91,0.59,0.48}
\definecolor{DarkSeaGreen1}{rgb}{0.76,1.00,0.76}
\definecolor{DarkSeaGreen2}{rgb}{0.71,0.93,0.71}
\definecolor{DarkSeaGreen3}{rgb}{0.61,0.80,0.61}
\definecolor{DarkSeaGreen4}{rgb}{0.41,0.55,0.41}
\definecolor{DarkSeaGreen}{rgb}{0.56,0.74,0.56}
\definecolor{DarkSlateBlue}{rgb}{0.28,0.24,0.55}
\definecolor{DarkSlateGray1}{rgb}{0.59,1.00,1.00}
\definecolor{DarkSlateGray2}{rgb}{0.55,0.93,0.93}
\definecolor{DarkSlateGray3}{rgb}{0.47,0.80,0.80}
\definecolor{DarkSlateGray4}{rgb}{0.32,0.55,0.55}
\definecolor{DarkSlateGray}{rgb}{0.18,0.31,0.31}
\definecolor{DarkSlateGrey}{rgb}{0.18,0.31,0.31}
\definecolor{DarkTurquoise}{rgb}{0.00,0.81,0.82}
\definecolor{DarkViolet}{rgb}{0.58,0.00,0.83}
\definecolor{DeepPink1}{rgb}{1.00,0.08,0.58}
\definecolor{DeepPink2}{rgb}{0.93,0.07,0.54}
\definecolor{DeepPink3}{rgb}{0.80,0.06,0.46}
\definecolor{DeepPink4}{rgb}{0.55,0.04,0.31}
\definecolor{DeepPink}{rgb}{1.00,0.08,0.58}
\definecolor{DeepSkyBlue1}{rgb}{0.00,0.75,1.00}
\definecolor{DeepSkyBlue2}{rgb}{0.00,0.70,0.93}
\definecolor{DeepSkyBlue3}{rgb}{0.00,0.60,0.80}
\definecolor{DeepSkyBlue4}{rgb}{0.00,0.41,0.55}
\definecolor{DeepSkyBlue}{rgb}{0.00,0.75,1.00}
\definecolor{DimGray}{rgb}{0.41,0.41,0.41}
\definecolor{DimGrey}{rgb}{0.41,0.41,0.41}
\definecolor{DodgerBlue1}{rgb}{0.12,0.56,1.00}
\definecolor{DodgerBlue2}{rgb}{0.11,0.53,0.93}
\definecolor{DodgerBlue3}{rgb}{0.09,0.45,0.80}
\definecolor{DodgerBlue4}{rgb}{0.06,0.31,0.55}
\definecolor{DodgerBlue}{rgb}{0.12,0.56,1.00}
\definecolor{FloralWhite}{rgb}{1.00,0.98,0.94}
\definecolor{ForestGreen}{rgb}{0.13,0.55,0.13}
\definecolor{GhostWhite}{rgb}{0.97,0.97,1.00}
\definecolor{GreenYellow}{rgb}{0.68,1.00,0.18}
\definecolor{HotPink1}{rgb}{1.00,0.43,0.71}
\definecolor{HotPink2}{rgb}{0.93,0.42,0.65}
\definecolor{HotPink3}{rgb}{0.80,0.38,0.56}
\definecolor{HotPink4}{rgb}{0.55,0.23,0.38}
\definecolor{HotPink}{rgb}{1.00,0.41,0.71}
\definecolor{IndianRed1}{rgb}{1.00,0.42,0.42}
\definecolor{IndianRed2}{rgb}{0.93,0.39,0.39}
\definecolor{IndianRed3}{rgb}{0.80,0.33,0.33}
\definecolor{IndianRed4}{rgb}{0.55,0.23,0.23}
\definecolor{IndianRed}{rgb}{0.80,0.36,0.36}
\definecolor{LavenderBlush1}{rgb}{1.00,0.94,0.96}
\definecolor{LavenderBlush2}{rgb}{0.93,0.88,0.90}
\definecolor{LavenderBlush3}{rgb}{0.80,0.76,0.77}
\definecolor{LavenderBlush4}{rgb}{0.55,0.51,0.53}
\definecolor{LavenderBlush}{rgb}{1.00,0.94,0.96}
\definecolor{LawnGreen}{rgb}{0.49,0.99,0.00}
\definecolor{LemonChiffon1}{rgb}{1.00,0.98,0.80}
\definecolor{LemonChiffon2}{rgb}{0.93,0.91,0.75}
\definecolor{LemonChiffon3}{rgb}{0.80,0.79,0.65}
\definecolor{LemonChiffon4}{rgb}{0.55,0.54,0.44}
\definecolor{LemonChiffon}{rgb}{1.00,0.98,0.80}
\definecolor{LightBlue1}{rgb}{0.75,0.94,1.00}
\definecolor{LightBlue2}{rgb}{0.70,0.87,0.93}
\definecolor{LightBlue3}{rgb}{0.60,0.75,0.80}
\definecolor{LightBlue4}{rgb}{0.41,0.51,0.55}
\definecolor{LightBlue}{rgb}{0.68,0.85,0.90}
\definecolor{LightCoral}{rgb}{0.94,0.50,0.50}
\definecolor{LightCyan1}{rgb}{0.88,1.00,1.00}
\definecolor{LightCyan2}{rgb}{0.82,0.93,0.93}
\definecolor{LightCyan3}{rgb}{0.71,0.80,0.80}
\definecolor{LightCyan4}{rgb}{0.48,0.55,0.55}
\definecolor{LightCyan}{rgb}{0.88,1.00,1.00}
\definecolor{LightGoldenrod1}{rgb}{1.00,0.93,0.55}
\definecolor{LightGoldenrod2}{rgb}{0.93,0.86,0.51}
\definecolor{LightGoldenrod3}{rgb}{0.80,0.75,0.44}
\definecolor{LightGoldenrod4}{rgb}{0.55,0.51,0.30}
\definecolor{LightGoldenrodYellow}{rgb}{0.98,0.98,0.82}
\definecolor{LightGoldenrod}{rgb}{0.93,0.87,0.51}
\definecolor{LightGray}{rgb}{0.83,0.83,0.83}
\definecolor{LightGreen}{rgb}{0.56,0.93,0.56}
\definecolor{LightGrey}{rgb}{0.83,0.83,0.83}
\definecolor{LightPink1}{rgb}{1.00,0.68,0.73}
\definecolor{LightPink2}{rgb}{0.93,0.64,0.68}
\definecolor{LightPink3}{rgb}{0.80,0.55,0.58}
\definecolor{LightPink4}{rgb}{0.55,0.37,0.40}
\definecolor{LightPink}{rgb}{1.00,0.71,0.76}
\definecolor{LightSalmon1}{rgb}{1.00,0.63,0.48}
\definecolor{LightSalmon2}{rgb}{0.93,0.58,0.45}
\definecolor{LightSalmon3}{rgb}{0.80,0.51,0.38}
\definecolor{LightSalmon4}{rgb}{0.55,0.34,0.26}
\definecolor{LightSalmon}{rgb}{1.00,0.63,0.48}
\definecolor{LightSeaGreen}{rgb}{0.13,0.70,0.67}
\definecolor{LightSkyBlue1}{rgb}{0.69,0.89,1.00}
\definecolor{LightSkyBlue2}{rgb}{0.64,0.83,0.93}
\definecolor{LightSkyBlue3}{rgb}{0.55,0.71,0.80}
\definecolor{LightSkyBlue4}{rgb}{0.38,0.48,0.55}
\definecolor{LightSkyBlue}{rgb}{0.53,0.81,0.98}
\definecolor{LightSlateBlue}{rgb}{0.52,0.44,1.00}
\definecolor{LightSlateGray}{rgb}{0.47,0.53,0.60}
\definecolor{LightSlateGrey}{rgb}{0.47,0.53,0.60}
\definecolor{LightSteelBlue1}{rgb}{0.79,0.88,1.00}
\definecolor{LightSteelBlue2}{rgb}{0.74,0.82,0.93}
\definecolor{LightSteelBlue3}{rgb}{0.64,0.71,0.80}
\definecolor{LightSteelBlue4}{rgb}{0.43,0.48,0.55}
\definecolor{LightSteelBlue}{rgb}{0.69,0.77,0.87}
\definecolor{LightYellow1}{rgb}{1.00,1.00,0.88}
\definecolor{LightYellow2}{rgb}{0.93,0.93,0.82}
\definecolor{LightYellow3}{rgb}{0.80,0.80,0.71}
\definecolor{LightYellow4}{rgb}{0.55,0.55,0.48}
\definecolor{LightYellow}{rgb}{1.00,1.00,0.88}
\definecolor{LimeGreen}{rgb}{0.20,0.80,0.20}
\definecolor{MediumAquamarine}{rgb}{0.40,0.80,0.67}
\definecolor{MediumBlue}{rgb}{0.00,0.00,0.80}
\definecolor{MediumOrchid1}{rgb}{0.88,0.40,1.00}
\definecolor{MediumOrchid2}{rgb}{0.82,0.37,0.93}
\definecolor{MediumOrchid3}{rgb}{0.71,0.32,0.80}
\definecolor{MediumOrchid4}{rgb}{0.48,0.22,0.55}
\definecolor{MediumOrchid}{rgb}{0.73,0.33,0.83}
\definecolor{MediumPurple1}{rgb}{0.67,0.51,1.00}
\definecolor{MediumPurple2}{rgb}{0.62,0.47,0.93}
\definecolor{MediumPurple3}{rgb}{0.54,0.41,0.80}
\definecolor{MediumPurple4}{rgb}{0.36,0.28,0.55}
\definecolor{MediumPurple}{rgb}{0.58,0.44,0.86}
\definecolor{MediumSeaGreen}{rgb}{0.24,0.70,0.44}
\definecolor{MediumSlateBlue}{rgb}{0.48,0.41,0.93}
\definecolor{MediumSpringGreen}{rgb}{0.00,0.98,0.60}
\definecolor{MediumTurquoise}{rgb}{0.28,0.82,0.80}
\definecolor{MediumVioletRed}{rgb}{0.78,0.08,0.52}
\definecolor{MidnightBlue}{rgb}{0.10,0.10,0.44}
\definecolor{MintCream}{rgb}{0.96,1.00,0.98}
\definecolor{MistyRose1}{rgb}{1.00,0.89,0.88}
\definecolor{MistyRose2}{rgb}{0.93,0.84,0.82}
\definecolor{MistyRose3}{rgb}{0.80,0.72,0.71}
\definecolor{MistyRose4}{rgb}{0.55,0.49,0.48}
\definecolor{MistyRose}{rgb}{1.00,0.89,0.88}
\definecolor{NavajoWhite1}{rgb}{1.00,0.87,0.68}
\definecolor{NavajoWhite2}{rgb}{0.93,0.81,0.63}
\definecolor{NavajoWhite3}{rgb}{0.80,0.70,0.55}
\definecolor{NavajoWhite4}{rgb}{0.55,0.47,0.37}
\definecolor{NavajoWhite}{rgb}{1.00,0.87,0.68}
\definecolor{NavyBlue}{rgb}{0.00,0.00,0.50}
\definecolor{OldLace}{rgb}{0.99,0.96,0.90}
\definecolor{OliveDrab1}{rgb}{0.75,1.00,0.24}
\definecolor{OliveDrab2}{rgb}{0.70,0.93,0.23}
\definecolor{OliveDrab3}{rgb}{0.60,0.80,0.20}
\definecolor{OliveDrab4}{rgb}{0.41,0.55,0.13}
\definecolor{OliveDrab}{rgb}{0.42,0.56,0.14}
\definecolor{OrangeRed1}{rgb}{1.00,0.27,0.00}
\definecolor{OrangeRed2}{rgb}{0.93,0.25,0.00}
\definecolor{OrangeRed3}{rgb}{0.80,0.22,0.00}
\definecolor{OrangeRed4}{rgb}{0.55,0.15,0.00}
\definecolor{OrangeRed}{rgb}{1.00,0.27,0.00}
\definecolor{PaleGoldenrod}{rgb}{0.93,0.91,0.67}
\definecolor{PaleGreen1}{rgb}{0.60,1.00,0.60}
\definecolor{PaleGreen2}{rgb}{0.56,0.93,0.56}
\definecolor{PaleGreen3}{rgb}{0.49,0.80,0.49}
\definecolor{PaleGreen4}{rgb}{0.33,0.55,0.33}
\definecolor{PaleGreen}{rgb}{0.60,0.98,0.60}
\definecolor{PaleTurquoise1}{rgb}{0.73,1.00,1.00}
\definecolor{PaleTurquoise2}{rgb}{0.68,0.93,0.93}
\definecolor{PaleTurquoise3}{rgb}{0.59,0.80,0.80}
\definecolor{PaleTurquoise4}{rgb}{0.40,0.55,0.55}
\definecolor{PaleTurquoise}{rgb}{0.69,0.93,0.93}
\definecolor{PaleVioletRed1}{rgb}{1.00,0.51,0.67}
\definecolor{PaleVioletRed2}{rgb}{0.93,0.47,0.62}
\definecolor{PaleVioletRed3}{rgb}{0.80,0.41,0.54}
\definecolor{PaleVioletRed4}{rgb}{0.55,0.28,0.36}
\definecolor{PaleVioletRed}{rgb}{0.86,0.44,0.58}
\definecolor{PapayaWhip}{rgb}{1.00,0.94,0.84}
\definecolor{PeachPuff1}{rgb}{1.00,0.85,0.73}
\definecolor{PeachPuff2}{rgb}{0.93,0.80,0.68}
\definecolor{PeachPuff3}{rgb}{0.80,0.69,0.58}
\definecolor{PeachPuff4}{rgb}{0.55,0.47,0.40}
\definecolor{PeachPuff}{rgb}{1.00,0.85,0.73}
\definecolor{PowderBlue}{rgb}{0.69,0.88,0.90}
\definecolor{RosyBrown1}{rgb}{1.00,0.76,0.76}
\definecolor{RosyBrown2}{rgb}{0.93,0.71,0.71}
\definecolor{RosyBrown3}{rgb}{0.80,0.61,0.61}
\definecolor{RosyBrown4}{rgb}{0.55,0.41,0.41}
\definecolor{RosyBrown}{rgb}{0.74,0.56,0.56}
\definecolor{RoyalBlue1}{rgb}{0.28,0.46,1.00}
\definecolor{RoyalBlue2}{rgb}{0.26,0.43,0.93}
\definecolor{RoyalBlue3}{rgb}{0.23,0.37,0.80}
\definecolor{RoyalBlue4}{rgb}{0.15,0.25,0.55}
\definecolor{RoyalBlue}{rgb}{0.25,0.41,0.88}
\definecolor{SaddleBrown}{rgb}{0.55,0.27,0.07}
\definecolor{SandyBrown}{rgb}{0.96,0.64,0.38}
\definecolor{SeaGreen1}{rgb}{0.33,1.00,0.62}
\definecolor{SeaGreen2}{rgb}{0.31,0.93,0.58}
\definecolor{SeaGreen3}{rgb}{0.26,0.80,0.50}
\definecolor{SeaGreen4}{rgb}{0.18,0.55,0.34}
\definecolor{SeaGreen}{rgb}{0.18,0.55,0.34}
\definecolor{SkyBlue1}{rgb}{0.53,0.81,1.00}
\definecolor{SkyBlue2}{rgb}{0.49,0.75,0.93}
\definecolor{SkyBlue3}{rgb}{0.42,0.65,0.80}
\definecolor{SkyBlue4}{rgb}{0.29,0.44,0.55}
\definecolor{SkyBlue}{rgb}{0.53,0.81,0.92}
\definecolor{SlateBlue1}{rgb}{0.51,0.44,1.00}
\definecolor{SlateBlue2}{rgb}{0.48,0.40,0.93}
\definecolor{SlateBlue3}{rgb}{0.41,0.35,0.80}
\definecolor{SlateBlue4}{rgb}{0.28,0.24,0.55}
\definecolor{SlateBlue}{rgb}{0.42,0.35,0.80}
\definecolor{SlateGray1}{rgb}{0.78,0.89,1.00}
\definecolor{SlateGray2}{rgb}{0.73,0.83,0.93}
\definecolor{SlateGray3}{rgb}{0.62,0.71,0.80}
\definecolor{SlateGray4}{rgb}{0.42,0.48,0.55}
\definecolor{SlateGray}{rgb}{0.44,0.50,0.56}
\definecolor{SlateGrey}{rgb}{0.44,0.50,0.56}
\definecolor{SpringGreen1}{rgb}{0.00,1.00,0.50}
\definecolor{SpringGreen2}{rgb}{0.00,0.93,0.46}
\definecolor{SpringGreen3}{rgb}{0.00,0.80,0.40}
\definecolor{SpringGreen4}{rgb}{0.00,0.55,0.27}
\definecolor{SpringGreen}{rgb}{0.00,1.00,0.50}
\definecolor{SteelBlue1}{rgb}{0.39,0.72,1.00}
\definecolor{SteelBlue2}{rgb}{0.36,0.67,0.93}
\definecolor{SteelBlue3}{rgb}{0.31,0.58,0.80}
\definecolor{SteelBlue4}{rgb}{0.21,0.39,0.55}
\definecolor{SteelBlue}{rgb}{0.27,0.51,0.71}
\definecolor{VioletRed1}{rgb}{1.00,0.24,0.59}
\definecolor{VioletRed2}{rgb}{0.93,0.23,0.55}
\definecolor{VioletRed3}{rgb}{0.80,0.20,0.47}
\definecolor{VioletRed4}{rgb}{0.55,0.13,0.32}
\definecolor{VioletRed}{rgb}{0.82,0.13,0.56}
\definecolor{WhiteSmoke}{rgb}{0.96,0.96,0.96}
\definecolor{YellowGreen}{rgb}{0.60,0.80,0.20}
\definecolor{aliceblue}{rgb}{0.94,0.97,1.00}
\definecolor{antiquewhite}{rgb}{0.98,0.92,0.84}
\definecolor{aquamarine1}{rgb}{0.50,1.00,0.83}
\definecolor{aquamarine2}{rgb}{0.46,0.93,0.78}
\definecolor{aquamarine3}{rgb}{0.40,0.80,0.67}
\definecolor{aquamarine4}{rgb}{0.27,0.55,0.45}
\definecolor{aquamarine}{rgb}{0.50,1.00,0.83}
\definecolor{azure1}{rgb}{0.94,1.00,1.00}
\definecolor{azure2}{rgb}{0.88,0.93,0.93}
\definecolor{azure3}{rgb}{0.76,0.80,0.80}
\definecolor{azure4}{rgb}{0.51,0.55,0.55}
\definecolor{azure}{rgb}{0.94,1.00,1.00}
\definecolor{beige}{rgb}{0.96,0.96,0.86}
\definecolor{bisque1}{rgb}{1.00,0.89,0.77}
\definecolor{bisque2}{rgb}{0.93,0.84,0.72}
\definecolor{bisque3}{rgb}{0.80,0.72,0.62}
\definecolor{bisque4}{rgb}{0.55,0.49,0.42}
\definecolor{bisque}{rgb}{1.00,0.89,0.77}
\definecolor{black}{rgb}{0.00,0.00,0.00}
\definecolor{blanchedalmond}{rgb}{1.00,0.92,0.80}
\definecolor{blue1}{rgb}{0.00,0.00,1.00}
\definecolor{blue2}{rgb}{0.00,0.00,0.93}
\definecolor{blue3}{rgb}{0.00,0.00,0.80}
\definecolor{blue4}{rgb}{0.00,0.00,0.55}
\definecolor{blueviolet}{rgb}{0.54,0.17,0.89}
\definecolor{blue}{rgb}{0.00,0.00,1.00}
\definecolor{brown1}{rgb}{1.00,0.25,0.25}
\definecolor{brown2}{rgb}{0.93,0.23,0.23}
\definecolor{brown3}{rgb}{0.80,0.20,0.20}
\definecolor{brown4}{rgb}{0.55,0.14,0.14}
\definecolor{brown}{rgb}{0.65,0.16,0.16}
\definecolor{burlywood1}{rgb}{1.00,0.83,0.61}
\definecolor{burlywood2}{rgb}{0.93,0.77,0.57}
\definecolor{burlywood3}{rgb}{0.80,0.67,0.49}
\definecolor{burlywood4}{rgb}{0.55,0.45,0.33}
\definecolor{burlywood}{rgb}{0.87,0.72,0.53}
\definecolor{cadetblue}{rgb}{0.37,0.62,0.63}
\definecolor{chartreuse1}{rgb}{0.50,1.00,0.00}
\definecolor{chartreuse2}{rgb}{0.46,0.93,0.00}
\definecolor{chartreuse3}{rgb}{0.40,0.80,0.00}
\definecolor{chartreuse4}{rgb}{0.27,0.55,0.00}
\definecolor{chartreuse}{rgb}{0.50,1.00,0.00}
\definecolor{chocolate1}{rgb}{1.00,0.50,0.14}
\definecolor{chocolate2}{rgb}{0.93,0.46,0.13}
\definecolor{chocolate3}{rgb}{0.80,0.40,0.11}
\definecolor{chocolate4}{rgb}{0.55,0.27,0.07}
\definecolor{chocolate}{rgb}{0.82,0.41,0.12}
\definecolor{coral1}{rgb}{1.00,0.45,0.34}
\definecolor{coral2}{rgb}{0.93,0.42,0.31}
\definecolor{coral3}{rgb}{0.80,0.36,0.27}
\definecolor{coral4}{rgb}{0.55,0.24,0.18}
\definecolor{coral}{rgb}{1.00,0.50,0.31}
\definecolor{cornflowerblue}{rgb}{0.39,0.58,0.93}
\definecolor{cornsilk1}{rgb}{1.00,0.97,0.86}
\definecolor{cornsilk2}{rgb}{0.93,0.91,0.80}
\definecolor{cornsilk3}{rgb}{0.80,0.78,0.69}
\definecolor{cornsilk4}{rgb}{0.55,0.53,0.47}
\definecolor{cornsilk}{rgb}{1.00,0.97,0.86}
\definecolor{cyan1}{rgb}{0.00,1.00,1.00}
\definecolor{cyan2}{rgb}{0.00,0.93,0.93}
\definecolor{cyan3}{rgb}{0.00,0.80,0.80}
\definecolor{cyan4}{rgb}{0.00,0.55,0.55}
\definecolor{cyan}{rgb}{0.00,1.00,1.00}
\definecolor{darkblue}{rgb}{0.00,0.00,0.55}
\definecolor{darkcyan}{rgb}{0.00,0.55,0.55}
\definecolor{darkgoldenrod}{rgb}{0.72,0.53,0.04}
\definecolor{darkgray}{rgb}{0.66,0.66,0.66}
\definecolor{darkgreen}{rgb}{0.00,0.39,0.00}
\definecolor{darkgrey}{rgb}{0.66,0.66,0.66}
\definecolor{darkkhaki}{rgb}{0.74,0.72,0.42}
\definecolor{darkmagenta}{rgb}{0.55,0.00,0.55}
\definecolor{darkolive}{rgb}{0.33,0.42,0.18}
\definecolor{darkorange}{rgb}{1.00,0.55,0.00}
\definecolor{darkorchid}{rgb}{0.60,0.20,0.80}
\definecolor{darkred}{rgb}{0.55,0.00,0.00}
\definecolor{darksalmon}{rgb}{0.91,0.59,0.48}
\definecolor{darksea}{rgb}{0.56,0.74,0.56}
\definecolor{darkslate}{rgb}{0.18,0.31,0.31}
\definecolor{darkslate}{rgb}{0.18,0.31,0.31}
\definecolor{darkslate}{rgb}{0.28,0.24,0.55}
\definecolor{darkturquoise}{rgb}{0.00,0.81,0.82}
\definecolor{darkviolet}{rgb}{0.58,0.00,0.83}
\definecolor{deeppink}{rgb}{1.00,0.08,0.58}
\definecolor{deepsky}{rgb}{0.00,0.75,1.00}
\definecolor{dimgray}{rgb}{0.41,0.41,0.41}
\definecolor{dimgrey}{rgb}{0.41,0.41,0.41}
\definecolor{dodgerblue}{rgb}{0.12,0.56,1.00}
\definecolor{firebrick1}{rgb}{1.00,0.19,0.19}
\definecolor{firebrick2}{rgb}{0.93,0.17,0.17}
\definecolor{firebrick3}{rgb}{0.80,0.15,0.15}
\definecolor{firebrick4}{rgb}{0.55,0.10,0.10}
\definecolor{firebrick}{rgb}{0.70,0.13,0.13}
\definecolor{floralwhite}{rgb}{1.00,0.98,0.94}
\definecolor{forestgreen}{rgb}{0.13,0.55,0.13}
\definecolor{gainsboro}{rgb}{0.86,0.86,0.86}
\definecolor{ghostwhite}{rgb}{0.97,0.97,1.00}
\definecolor{gold1}{rgb}{1.00,0.84,0.00}
\definecolor{gold2}{rgb}{0.93,0.79,0.00}
\definecolor{gold3}{rgb}{0.80,0.68,0.00}
\definecolor{gold4}{rgb}{0.55,0.46,0.00}
\definecolor{goldenrod1}{rgb}{1.00,0.76,0.15}
\definecolor{goldenrod2}{rgb}{0.93,0.71,0.13}
\definecolor{goldenrod3}{rgb}{0.80,0.61,0.11}
\definecolor{goldenrod4}{rgb}{0.55,0.41,0.08}
\definecolor{goldenrod}{rgb}{0.85,0.65,0.13}
\definecolor{gold}{rgb}{1.00,0.84,0.00}
\definecolor{gray0}{rgb}{0.00,0.00,0.00}
\definecolor{gray100}{rgb}{1.00,1.00,1.00}
\definecolor{gray10}{rgb}{0.10,0.10,0.10}
\definecolor{gray11}{rgb}{0.11,0.11,0.11}
\definecolor{gray12}{rgb}{0.12,0.12,0.12}
\definecolor{gray13}{rgb}{0.13,0.13,0.13}
\definecolor{gray14}{rgb}{0.14,0.14,0.14}
\definecolor{gray15}{rgb}{0.15,0.15,0.15}
\definecolor{gray16}{rgb}{0.16,0.16,0.16}
\definecolor{gray17}{rgb}{0.17,0.17,0.17}
\definecolor{gray18}{rgb}{0.18,0.18,0.18}
\definecolor{gray19}{rgb}{0.19,0.19,0.19}
\definecolor{gray1}{rgb}{0.01,0.01,0.01}
\definecolor{gray20}{rgb}{0.20,0.20,0.20}
\definecolor{gray21}{rgb}{0.21,0.21,0.21}
\definecolor{gray22}{rgb}{0.22,0.22,0.22}
\definecolor{gray23}{rgb}{0.23,0.23,0.23}
\definecolor{gray24}{rgb}{0.24,0.24,0.24}
\definecolor{gray25}{rgb}{0.25,0.25,0.25}
\definecolor{gray26}{rgb}{0.26,0.26,0.26}
\definecolor{gray27}{rgb}{0.27,0.27,0.27}
\definecolor{gray28}{rgb}{0.28,0.28,0.28}
\definecolor{gray29}{rgb}{0.29,0.29,0.29}
\definecolor{gray2}{rgb}{0.02,0.02,0.02}
\definecolor{gray30}{rgb}{0.30,0.30,0.30}
\definecolor{gray31}{rgb}{0.31,0.31,0.31}
\definecolor{gray32}{rgb}{0.32,0.32,0.32}
\definecolor{gray33}{rgb}{0.33,0.33,0.33}
\definecolor{gray34}{rgb}{0.34,0.34,0.34}
\definecolor{gray35}{rgb}{0.35,0.35,0.35}
\definecolor{gray36}{rgb}{0.36,0.36,0.36}
\definecolor{gray37}{rgb}{0.37,0.37,0.37}
\definecolor{gray38}{rgb}{0.38,0.38,0.38}
\definecolor{gray39}{rgb}{0.39,0.39,0.39}
\definecolor{gray3}{rgb}{0.03,0.03,0.03}
\definecolor{gray40}{rgb}{0.40,0.40,0.40}
\definecolor{gray41}{rgb}{0.41,0.41,0.41}
\definecolor{gray42}{rgb}{0.42,0.42,0.42}
\definecolor{gray43}{rgb}{0.43,0.43,0.43}
\definecolor{gray44}{rgb}{0.44,0.44,0.44}
\definecolor{gray45}{rgb}{0.45,0.45,0.45}
\definecolor{gray46}{rgb}{0.46,0.46,0.46}
\definecolor{gray47}{rgb}{0.47,0.47,0.47}
\definecolor{gray48}{rgb}{0.48,0.48,0.48}
\definecolor{gray49}{rgb}{0.49,0.49,0.49}
\definecolor{gray4}{rgb}{0.04,0.04,0.04}
\definecolor{gray50}{rgb}{0.50,0.50,0.50}
\definecolor{gray51}{rgb}{0.51,0.51,0.51}
\definecolor{gray52}{rgb}{0.52,0.52,0.52}
\definecolor{gray53}{rgb}{0.53,0.53,0.53}
\definecolor{gray54}{rgb}{0.54,0.54,0.54}
\definecolor{gray55}{rgb}{0.55,0.55,0.55}
\definecolor{gray56}{rgb}{0.56,0.56,0.56}
\definecolor{gray57}{rgb}{0.57,0.57,0.57}
\definecolor{gray58}{rgb}{0.58,0.58,0.58}
\definecolor{gray59}{rgb}{0.59,0.59,0.59}
\definecolor{gray5}{rgb}{0.05,0.05,0.05}
\definecolor{gray60}{rgb}{0.60,0.60,0.60}
\definecolor{gray61}{rgb}{0.61,0.61,0.61}
\definecolor{gray62}{rgb}{0.62,0.62,0.62}
\definecolor{gray63}{rgb}{0.63,0.63,0.63}
\definecolor{gray64}{rgb}{0.64,0.64,0.64}
\definecolor{gray65}{rgb}{0.65,0.65,0.65}
\definecolor{gray66}{rgb}{0.66,0.66,0.66}
\definecolor{gray67}{rgb}{0.67,0.67,0.67}
\definecolor{gray68}{rgb}{0.68,0.68,0.68}
\definecolor{gray69}{rgb}{0.69,0.69,0.69}
\definecolor{gray6}{rgb}{0.06,0.06,0.06}
\definecolor{gray70}{rgb}{0.70,0.70,0.70}
\definecolor{gray71}{rgb}{0.71,0.71,0.71}
\definecolor{gray72}{rgb}{0.72,0.72,0.72}
\definecolor{gray73}{rgb}{0.73,0.73,0.73}
\definecolor{gray74}{rgb}{0.74,0.74,0.74}
\definecolor{gray75}{rgb}{0.75,0.75,0.75}
\definecolor{gray76}{rgb}{0.76,0.76,0.76}
\definecolor{gray77}{rgb}{0.77,0.77,0.77}
\definecolor{gray78}{rgb}{0.78,0.78,0.78}
\definecolor{gray79}{rgb}{0.79,0.79,0.79}
\definecolor{gray7}{rgb}{0.07,0.07,0.07}
\definecolor{gray80}{rgb}{0.80,0.80,0.80}
\definecolor{gray81}{rgb}{0.81,0.81,0.81}
\definecolor{gray82}{rgb}{0.82,0.82,0.82}
\definecolor{gray83}{rgb}{0.83,0.83,0.83}
\definecolor{gray84}{rgb}{0.84,0.84,0.84}
\definecolor{gray85}{rgb}{0.85,0.85,0.85}
\definecolor{gray86}{rgb}{0.86,0.86,0.86}
\definecolor{gray87}{rgb}{0.87,0.87,0.87}
\definecolor{gray88}{rgb}{0.88,0.88,0.88}
\definecolor{gray89}{rgb}{0.89,0.89,0.89}
\definecolor{gray8}{rgb}{0.08,0.08,0.08}
\definecolor{gray90}{rgb}{0.90,0.90,0.90}
\definecolor{gray91}{rgb}{0.91,0.91,0.91}
\definecolor{gray92}{rgb}{0.92,0.92,0.92}
\definecolor{gray93}{rgb}{0.93,0.93,0.93}
\definecolor{gray94}{rgb}{0.94,0.94,0.94}
\definecolor{gray95}{rgb}{0.95,0.95,0.95}
\definecolor{gray96}{rgb}{0.96,0.96,0.96}
\definecolor{gray97}{rgb}{0.97,0.97,0.97}
\definecolor{gray98}{rgb}{0.98,0.98,0.98}
\definecolor{gray99}{rgb}{0.99,0.99,0.99}
\definecolor{gray9}{rgb}{0.09,0.09,0.09}
\definecolor{gray}{rgb}{0.75,0.75,0.75}
\definecolor{green1}{rgb}{0.00,1.00,0.00}
\definecolor{green2}{rgb}{0.00,0.93,0.00}
\definecolor{green3}{rgb}{0.00,0.80,0.00}
\definecolor{green4}{rgb}{0.00,0.55,0.00}
\definecolor{greenyellow}{rgb}{0.68,1.00,0.18}
\definecolor{green}{rgb}{0.00,1.00,0.00}
\definecolor{grey0}{rgb}{0.00,0.00,0.00}
\definecolor{grey100}{rgb}{1.00,1.00,1.00}
\definecolor{grey10}{rgb}{0.10,0.10,0.10}
\definecolor{grey11}{rgb}{0.11,0.11,0.11}
\definecolor{grey12}{rgb}{0.12,0.12,0.12}
\definecolor{grey13}{rgb}{0.13,0.13,0.13}
\definecolor{grey14}{rgb}{0.14,0.14,0.14}
\definecolor{grey15}{rgb}{0.15,0.15,0.15}
\definecolor{grey16}{rgb}{0.16,0.16,0.16}
\definecolor{grey17}{rgb}{0.17,0.17,0.17}
\definecolor{grey18}{rgb}{0.18,0.18,0.18}
\definecolor{grey19}{rgb}{0.19,0.19,0.19}
\definecolor{grey1}{rgb}{0.01,0.01,0.01}
\definecolor{grey20}{rgb}{0.20,0.20,0.20}
\definecolor{grey21}{rgb}{0.21,0.21,0.21}
\definecolor{grey22}{rgb}{0.22,0.22,0.22}
\definecolor{grey23}{rgb}{0.23,0.23,0.23}
\definecolor{grey24}{rgb}{0.24,0.24,0.24}
\definecolor{grey25}{rgb}{0.25,0.25,0.25}
\definecolor{grey26}{rgb}{0.26,0.26,0.26}
\definecolor{grey27}{rgb}{0.27,0.27,0.27}
\definecolor{grey28}{rgb}{0.28,0.28,0.28}
\definecolor{grey29}{rgb}{0.29,0.29,0.29}
\definecolor{grey2}{rgb}{0.02,0.02,0.02}
\definecolor{grey30}{rgb}{0.30,0.30,0.30}
\definecolor{grey31}{rgb}{0.31,0.31,0.31}
\definecolor{grey32}{rgb}{0.32,0.32,0.32}
\definecolor{grey33}{rgb}{0.33,0.33,0.33}
\definecolor{grey34}{rgb}{0.34,0.34,0.34}
\definecolor{grey35}{rgb}{0.35,0.35,0.35}
\definecolor{grey36}{rgb}{0.36,0.36,0.36}
\definecolor{grey37}{rgb}{0.37,0.37,0.37}
\definecolor{grey38}{rgb}{0.38,0.38,0.38}
\definecolor{grey39}{rgb}{0.39,0.39,0.39}
\definecolor{grey3}{rgb}{0.03,0.03,0.03}
\definecolor{grey40}{rgb}{0.40,0.40,0.40}
\definecolor{grey41}{rgb}{0.41,0.41,0.41}
\definecolor{grey42}{rgb}{0.42,0.42,0.42}
\definecolor{grey43}{rgb}{0.43,0.43,0.43}
\definecolor{grey44}{rgb}{0.44,0.44,0.44}
\definecolor{grey45}{rgb}{0.45,0.45,0.45}
\definecolor{grey46}{rgb}{0.46,0.46,0.46}
\definecolor{grey47}{rgb}{0.47,0.47,0.47}
\definecolor{grey48}{rgb}{0.48,0.48,0.48}
\definecolor{grey49}{rgb}{0.49,0.49,0.49}
\definecolor{grey4}{rgb}{0.04,0.04,0.04}
\definecolor{grey50}{rgb}{0.50,0.50,0.50}
\definecolor{grey51}{rgb}{0.51,0.51,0.51}
\definecolor{grey52}{rgb}{0.52,0.52,0.52}
\definecolor{grey53}{rgb}{0.53,0.53,0.53}
\definecolor{grey54}{rgb}{0.54,0.54,0.54}
\definecolor{grey55}{rgb}{0.55,0.55,0.55}
\definecolor{grey56}{rgb}{0.56,0.56,0.56}
\definecolor{grey57}{rgb}{0.57,0.57,0.57}
\definecolor{grey58}{rgb}{0.58,0.58,0.58}
\definecolor{grey59}{rgb}{0.59,0.59,0.59}
\definecolor{grey5}{rgb}{0.05,0.05,0.05}
\definecolor{grey60}{rgb}{0.60,0.60,0.60}
\definecolor{grey61}{rgb}{0.61,0.61,0.61}
\definecolor{grey62}{rgb}{0.62,0.62,0.62}
\definecolor{grey63}{rgb}{0.63,0.63,0.63}
\definecolor{grey64}{rgb}{0.64,0.64,0.64}
\definecolor{grey65}{rgb}{0.65,0.65,0.65}
\definecolor{grey66}{rgb}{0.66,0.66,0.66}
\definecolor{grey67}{rgb}{0.67,0.67,0.67}
\definecolor{grey68}{rgb}{0.68,0.68,0.68}
\definecolor{grey69}{rgb}{0.69,0.69,0.69}
\definecolor{grey6}{rgb}{0.06,0.06,0.06}
\definecolor{grey70}{rgb}{0.70,0.70,0.70}
\definecolor{grey71}{rgb}{0.71,0.71,0.71}
\definecolor{grey72}{rgb}{0.72,0.72,0.72}
\definecolor{grey73}{rgb}{0.73,0.73,0.73}
\definecolor{grey74}{rgb}{0.74,0.74,0.74}
\definecolor{grey75}{rgb}{0.75,0.75,0.75}
\definecolor{grey76}{rgb}{0.76,0.76,0.76}
\definecolor{grey77}{rgb}{0.77,0.77,0.77}
\definecolor{grey78}{rgb}{0.78,0.78,0.78}
\definecolor{grey79}{rgb}{0.79,0.79,0.79}
\definecolor{grey7}{rgb}{0.07,0.07,0.07}
\definecolor{grey80}{rgb}{0.80,0.80,0.80}
\definecolor{grey81}{rgb}{0.81,0.81,0.81}
\definecolor{grey82}{rgb}{0.82,0.82,0.82}
\definecolor{grey83}{rgb}{0.83,0.83,0.83}
\definecolor{grey84}{rgb}{0.84,0.84,0.84}
\definecolor{grey85}{rgb}{0.85,0.85,0.85}
\definecolor{grey86}{rgb}{0.86,0.86,0.86}
\definecolor{grey87}{rgb}{0.87,0.87,0.87}
\definecolor{grey88}{rgb}{0.88,0.88,0.88}
\definecolor{grey89}{rgb}{0.89,0.89,0.89}
\definecolor{grey8}{rgb}{0.08,0.08,0.08}
\definecolor{grey90}{rgb}{0.90,0.90,0.90}
\definecolor{grey91}{rgb}{0.91,0.91,0.91}
\definecolor{grey92}{rgb}{0.92,0.92,0.92}
\definecolor{grey93}{rgb}{0.93,0.93,0.93}
\definecolor{grey94}{rgb}{0.94,0.94,0.94}
\definecolor{grey95}{rgb}{0.95,0.95,0.95}
\definecolor{grey96}{rgb}{0.96,0.96,0.96}
\definecolor{grey97}{rgb}{0.97,0.97,0.97}
\definecolor{grey98}{rgb}{0.98,0.98,0.98}
\definecolor{grey99}{rgb}{0.99,0.99,0.99}
\definecolor{grey9}{rgb}{0.09,0.09,0.09}
\definecolor{grey}{rgb}{0.75,0.75,0.75}
\definecolor{honeydew1}{rgb}{0.94,1.00,0.94}
\definecolor{honeydew2}{rgb}{0.88,0.93,0.88}
\definecolor{honeydew3}{rgb}{0.76,0.80,0.76}
\definecolor{honeydew4}{rgb}{0.51,0.55,0.51}
\definecolor{honeydew}{rgb}{0.94,1.00,0.94}
\definecolor{hotpink}{rgb}{1.00,0.41,0.71}
\definecolor{indianred}{rgb}{0.80,0.36,0.36}
\definecolor{ivory1}{rgb}{1.00,1.00,0.94}
\definecolor{ivory2}{rgb}{0.93,0.93,0.88}
\definecolor{ivory3}{rgb}{0.80,0.80,0.76}
\definecolor{ivory4}{rgb}{0.55,0.55,0.51}
\definecolor{ivory}{rgb}{1.00,1.00,0.94}
\definecolor{khaki1}{rgb}{1.00,0.96,0.56}
\definecolor{khaki2}{rgb}{0.93,0.90,0.52}
\definecolor{khaki3}{rgb}{0.80,0.78,0.45}
\definecolor{khaki4}{rgb}{0.55,0.53,0.31}
\definecolor{khaki}{rgb}{0.94,0.90,0.55}
\definecolor{lavenderblush}{rgb}{1.00,0.94,0.96}
\definecolor{lavender}{rgb}{0.90,0.90,0.98}
\definecolor{lawngreen}{rgb}{0.49,0.99,0.00}
\definecolor{lemonchiffon}{rgb}{1.00,0.98,0.80}
\definecolor{lightblue}{rgb}{0.68,0.85,0.90}
\definecolor{lightcoral}{rgb}{0.94,0.50,0.50}
\definecolor{lightcyan}{rgb}{0.88,1.00,1.00}
\definecolor{lightgoldenrod}{rgb}{0.93,0.87,0.51}
\definecolor{lightgoldenrod}{rgb}{0.98,0.98,0.82}
\definecolor{lightgray}{rgb}{0.83,0.83,0.83}
\definecolor{lightgreen}{rgb}{0.56,0.93,0.56}
\definecolor{lightgrey}{rgb}{0.83,0.83,0.83}
\definecolor{lightpink}{rgb}{1.00,0.71,0.76}
\definecolor{lightsalmon}{rgb}{1.00,0.63,0.48}
\definecolor{lightsea}{rgb}{0.13,0.70,0.67}
\definecolor{lightsky}{rgb}{0.53,0.81,0.98}
\definecolor{lightslate}{rgb}{0.47,0.53,0.60}
\definecolor{lightslate}{rgb}{0.47,0.53,0.60}
\definecolor{lightslate}{rgb}{0.52,0.44,1.00}
\definecolor{lightsteel}{rgb}{0.69,0.77,0.87}
\definecolor{lightyellow}{rgb}{1.00,1.00,0.88}
\definecolor{limegreen}{rgb}{0.20,0.80,0.20}
\definecolor{linen}{rgb}{0.98,0.94,0.90}
\definecolor{magenta1}{rgb}{1.00,0.00,1.00}
\definecolor{magenta2}{rgb}{0.93,0.00,0.93}
\definecolor{magenta3}{rgb}{0.80,0.00,0.80}
\definecolor{magenta4}{rgb}{0.55,0.00,0.55}
\definecolor{magenta}{rgb}{1.00,0.00,1.00}
\definecolor{maroon1}{rgb}{1.00,0.20,0.70}
\definecolor{maroon2}{rgb}{0.93,0.19,0.65}
\definecolor{maroon3}{rgb}{0.80,0.16,0.56}
\definecolor{maroon4}{rgb}{0.55,0.11,0.38}
\definecolor{maroon}{rgb}{0.69,0.19,0.38}
\definecolor{mediumaquamarine}{rgb}{0.40,0.80,0.67}
\definecolor{mediumblue}{rgb}{0.00,0.00,0.80}
\definecolor{mediumorchid}{rgb}{0.73,0.33,0.83}
\definecolor{mediumpurple}{rgb}{0.58,0.44,0.86}
\definecolor{mediumsea}{rgb}{0.24,0.70,0.44}
\definecolor{mediumslate}{rgb}{0.48,0.41,0.93}
\definecolor{mediumspring}{rgb}{0.00,0.98,0.60}
\definecolor{mediumturquoise}{rgb}{0.28,0.82,0.80}
\definecolor{mediumviolet}{rgb}{0.78,0.08,0.52}
\definecolor{midnightblue}{rgb}{0.10,0.10,0.44}
\definecolor{mintcream}{rgb}{0.96,1.00,0.98}
\definecolor{mistyrose}{rgb}{1.00,0.89,0.88}
\definecolor{moccasin}{rgb}{1.00,0.89,0.71}
\definecolor{navajowhite}{rgb}{1.00,0.87,0.68}
\definecolor{navyblue}{rgb}{0.00,0.00,0.50}
\definecolor{navy}{rgb}{0.00,0.00,0.50}
\definecolor{oldlace}{rgb}{0.99,0.96,0.90}
\definecolor{olivedrab}{rgb}{0.42,0.56,0.14}
\definecolor{orange1}{rgb}{1.00,0.65,0.00}
\definecolor{orange2}{rgb}{0.93,0.60,0.00}
\definecolor{orange3}{rgb}{0.80,0.52,0.00}
\definecolor{orange4}{rgb}{0.55,0.35,0.00}
\definecolor{orangered}{rgb}{1.00,0.27,0.00}
\definecolor{orange}{rgb}{1.00,0.65,0.00}
\definecolor{orchid1}{rgb}{1.00,0.51,0.98}
\definecolor{orchid2}{rgb}{0.93,0.48,0.91}
\definecolor{orchid3}{rgb}{0.80,0.41,0.79}
\definecolor{orchid4}{rgb}{0.55,0.28,0.54}
\definecolor{orchid}{rgb}{0.85,0.44,0.84}
\definecolor{palegoldenrod}{rgb}{0.93,0.91,0.67}
\definecolor{palegreen}{rgb}{0.60,0.98,0.60}
\definecolor{paleturquoise}{rgb}{0.69,0.93,0.93}
\definecolor{paleviolet}{rgb}{0.86,0.44,0.58}
\definecolor{papayawhip}{rgb}{1.00,0.94,0.84}
\definecolor{peachpuff}{rgb}{1.00,0.85,0.73}
\definecolor{peru}{rgb}{0.80,0.52,0.25}
\definecolor{pink1}{rgb}{1.00,0.71,0.77}
\definecolor{pink2}{rgb}{0.93,0.66,0.72}
\definecolor{pink3}{rgb}{0.80,0.57,0.62}
\definecolor{pink4}{rgb}{0.55,0.39,0.42}
\definecolor{pink}{rgb}{1.00,0.75,0.80}
\definecolor{plum1}{rgb}{1.00,0.73,1.00}
\definecolor{plum2}{rgb}{0.93,0.68,0.93}
\definecolor{plum3}{rgb}{0.80,0.59,0.80}
\definecolor{plum4}{rgb}{0.55,0.40,0.55}
\definecolor{plum}{rgb}{0.87,0.63,0.87}
\definecolor{powderblue}{rgb}{0.69,0.88,0.90}
\definecolor{purple1}{rgb}{0.61,0.19,1.00}
\definecolor{purple2}{rgb}{0.57,0.17,0.93}
\definecolor{purple3}{rgb}{0.49,0.15,0.80}
\definecolor{purple4}{rgb}{0.33,0.10,0.55}
\definecolor{purple}{rgb}{0.63,0.13,0.94}
\definecolor{red1}{rgb}{1.00,0.00,0.00}
\definecolor{red2}{rgb}{0.93,0.00,0.00}
\definecolor{red3}{rgb}{0.80,0.00,0.00}
\definecolor{red4}{rgb}{0.55,0.00,0.00}
\definecolor{red}{rgb}{1.00,0.00,0.00}
\definecolor{rosybrown}{rgb}{0.74,0.56,0.56}
\definecolor{royalblue}{rgb}{0.25,0.41,0.88}
\definecolor{saddlebrown}{rgb}{0.55,0.27,0.07}
\definecolor{salmon1}{rgb}{1.00,0.55,0.41}
\definecolor{salmon2}{rgb}{0.93,0.51,0.38}
\definecolor{salmon3}{rgb}{0.80,0.44,0.33}
\definecolor{salmon4}{rgb}{0.55,0.30,0.22}
\definecolor{salmon}{rgb}{0.98,0.50,0.45}
\definecolor{sandybrown}{rgb}{0.96,0.64,0.38}
\definecolor{seagreen}{rgb}{0.18,0.55,0.34}
\definecolor{seashell1}{rgb}{1.00,0.96,0.93}
\definecolor{seashell2}{rgb}{0.93,0.90,0.87}
\definecolor{seashell3}{rgb}{0.80,0.77,0.75}
\definecolor{seashell4}{rgb}{0.55,0.53,0.51}
\definecolor{seashell}{rgb}{1.00,0.96,0.93}
\definecolor{sienna1}{rgb}{1.00,0.51,0.28}
\definecolor{sienna2}{rgb}{0.93,0.47,0.26}
\definecolor{sienna3}{rgb}{0.80,0.41,0.22}
\definecolor{sienna4}{rgb}{0.55,0.28,0.15}
\definecolor{sienna}{rgb}{0.63,0.32,0.18}
\definecolor{skyblue}{rgb}{0.53,0.81,0.92}
\definecolor{slateblue}{rgb}{0.42,0.35,0.80}
\definecolor{slategray}{rgb}{0.44,0.50,0.56}
\definecolor{slategrey}{rgb}{0.44,0.50,0.56}
\definecolor{snow1}{rgb}{1.00,0.98,0.98}
\definecolor{snow2}{rgb}{0.93,0.91,0.91}
\definecolor{snow3}{rgb}{0.80,0.79,0.79}
\definecolor{snow4}{rgb}{0.55,0.54,0.54}
\definecolor{snow}{rgb}{1.00,0.98,0.98}
\definecolor{springgreen}{rgb}{0.00,1.00,0.50}
\definecolor{steelblue}{rgb}{0.27,0.51,0.71}
\definecolor{tan1}{rgb}{1.00,0.65,0.31}
\definecolor{tan2}{rgb}{0.93,0.60,0.29}
\definecolor{tan3}{rgb}{0.80,0.52,0.25}
\definecolor{tan4}{rgb}{0.55,0.35,0.17}
\definecolor{tan}{rgb}{0.82,0.71,0.55}
\definecolor{thistle1}{rgb}{1.00,0.88,1.00}
\definecolor{thistle2}{rgb}{0.93,0.82,0.93}
\definecolor{thistle3}{rgb}{0.80,0.71,0.80}
\definecolor{thistle4}{rgb}{0.55,0.48,0.55}
\definecolor{thistle}{rgb}{0.85,0.75,0.85}
\definecolor{tomato1}{rgb}{1.00,0.39,0.28}
\definecolor{tomato2}{rgb}{0.93,0.36,0.26}
\definecolor{tomato3}{rgb}{0.80,0.31,0.22}
\definecolor{tomato4}{rgb}{0.55,0.21,0.15}
\definecolor{tomato}{rgb}{1.00,0.39,0.28}
\definecolor{turquoise1}{rgb}{0.00,0.96,1.00}
\definecolor{turquoise2}{rgb}{0.00,0.90,0.93}
\definecolor{turquoise3}{rgb}{0.00,0.77,0.80}
\definecolor{turquoise4}{rgb}{0.00,0.53,0.55}
\definecolor{turquoise}{rgb}{0.25,0.88,0.82}
\definecolor{violetred}{rgb}{0.82,0.13,0.56}
\definecolor{violet}{rgb}{0.93,0.51,0.93}
\definecolor{wheat1}{rgb}{1.00,0.91,0.73}
\definecolor{wheat2}{rgb}{0.93,0.85,0.68}
\definecolor{wheat3}{rgb}{0.80,0.73,0.59}
\definecolor{wheat4}{rgb}{0.55,0.49,0.40}
\definecolor{wheat}{rgb}{0.96,0.87,0.70}
\definecolor{whitesmoke}{rgb}{0.96,0.96,0.96}
\definecolor{white}{rgb}{1.00,1.00,1.00}
\definecolor{yellow1}{rgb}{1.00,1.00,0.00}
\definecolor{yellow2}{rgb}{0.93,0.93,0.00}
\definecolor{yellow3}{rgb}{0.80,0.80,0.00}
\definecolor{yellow4}{rgb}{0.55,0.55,0.00}
\definecolor{yellowgreen}{rgb}{0.60,0.80,0.20}
\definecolor{yellow}{rgb}{1.00,1.00,0.00}

